Sampling in BV-Type Spaces

The sampling of functions of bounded variation (BV) is a long-standing problem in op- timization. The ability to sample such functions has relevance in the field of variational inverse problems, where the standard theory fails to guarantee the mere existence of solutions when the loss functional involves samples of BV functions. In this paper, we prove the continuity of sampling functionals and show that the differential operator D admits a unique local inverse. This canonical inversion enables us to formulate an existence theorem for a class of regularized optimization problems that incorporate samples of BV functions. Finally, we characterize the solution set in terms of its extreme points.

==> Sections/Section5/Section5.3.tex <==

\begin{Theorem}
\label{th:weakRT}
Assume that Assumptions 1 to 3 hold. 

If $\alpha<0$, $\,\omega=1,$ and the underlying system $(\bb{p},\bm{\iota})$ is the unique causal fundamental system, then
\begin{itemize}
    \item if $\lambda_2<\lambda_1$, then there exists a unique solution, of the form 
    \begin{equation}
        \mathcal{V}_\omega(\K)=\bigg\{a\frac{(\cdot-t_1)^{N-1}\e^{\alpha(\cdot-t_1)}}{(N-1)!}+\sum_{m=2}^Ma_mg_{\Ls}(\cdot-t_m)\bigg\}
    \end{equation}
    \item if $\lambda_2>\lambda_1$, then there exists a unique solution, of the form 
    \begin{equation}
        \mathcal{V}_\omega(\K)=\bigg\{\sum_{m=1}^Ma_mg_{\Ls}(\cdot-t_m)\bigg\}
    \end{equation}
    \item if $\lambda_2=\lambda_1$, then the solution set is a closed line, of the form 
    \begin{multline}
        \mathcal{V}_\omega(\K)=\bigg\{\theta a\frac{(\cdot-t_1)^{N-1}\e^{\alpha(\cdot-t_1)}}{(N-1)!}+(1-\theta)a_1g_{\Ls}(\cdot-t_1)\\+\sum_{m=2}^Ma_mg_{\Ls}(\cdot-t_m),\quad\theta\in[0,1]\bigg\}
    \end{multline}
\end{itemize}

If $\alpha>0$, $\,\omega=0,$ and the underlying system $(\bb{p},\bm{\iota})$ is the unique anti-causal fundamental system, then a symmetric result holds, where $g_{\Ls}$ in [?] is replaced by the anti-causal Green's function $\tilde g_{\Ls}.$
\begin{itemize}
    \item if $\lambda_2<\lambda_1$, then there exists a unique solution, of the form 
    \begin{equation}
        \mathcal{V}_\omega(\K)=\bigg\{a\frac{(\cdot-t_M)^{N-1}\e^{\alpha(\cdot-t_M)}}{(N-1)!}+\sum_{m=1}^{M-1}a_m\tilde g_{\Ls}(\cdot-t_m)\bigg\}
    \end{equation}
    \item if $\lambda_2>\lambda_1$, then there exists a unique solution, of the form 
    \begin{equation}
        \mathcal{V}_\omega(\K)=\bigg\{\sum_{m=1}^Ma_m\tilde g_{\Ls}(\cdot-t_m)\bigg\}
    \end{equation}
    \item if $\lambda_2=\lambda_1$, then the solution set is a closed line, of the form 
    \begin{multline}
        \mathcal{V}_\omega(\K)=\bigg\{\theta a\frac{(\cdot-t_M)^{N-1}\e^{\alpha(\cdot-t_M)}}{(N-1)!}+(1-\theta)a_M\tilde g_{\Ls}(\cdot-t_M)\\
        +\sum_{m=1}^{M-1}a_m\tilde g_{\Ls}(\cdot-t_m),\quad\theta\in[0,1]\bigg\}
    \end{multline}
\end{itemize}
\end{Theorem}

[COMMENTS]
\begin{itemize}
    \item how hard is unicity to get
    \item why $\alpha<0$ diff from $\alpha>0$ and $\alpha=0$
    \item what to do with other limits
\end{itemize}

\begin{proof}[\textbf{Proof of Theorem \ref{th:weakRT}}]
\hfill\\
Let $f=p+(g_{\Ls}\ast\mu)\in\M_{\Ls}(\K)$ and 
\begin{equation}
    \tilde f = p+(g_{\Ls}\ast\tilde{\mu}),\quad\text{with}\quad \tilde{\mu}=\mu(\{t_1\})\delta_{t_1}+\sum_{m=2}^{M}c_m\delta_{t_m},
\end{equation}
and 
\begin{equation}
    c_m=\int_{]t_{m-1},t_{m}]}\e^{\alpha(t_m-x)}\,\mathrm{d}\mu(x)
\end{equation}
Observe that 
\begin{equation}
\label{eq:4.2.105}
    \norm{\Ls\{\tilde f\}}_{\M}\leq\norm{\Ls\{f\}}_{\M}
\end{equation}
and that, because 
\begin{equation}
    \e^{\alpha(t_m+\epsilon-x)}<1\quad\text{over}\quad]t_m,t_{m+1}[,
\end{equation}
if $\mathrm{supp}(\mu)\nsubseteq\{t_m\}_{m=1}^M$, then the inequality in \eqref{eq:4.2.105} is strict. Next, we claim
\begin{equation}
\label{eq:4.2.107}
    \langle(\Dd-\alpha\I)^{N-1,\star}\{\bm{\delta}_{\bb{t}}^+\},\tilde f\rangle=\langle(\Dd-\alpha\I)^{N-1,\star}\{\bm{\delta}_{\bb{t}}^+\},f\rangle.
\end{equation}
Observe that \eqref{eq:4.2.107} is equivalent to, $\forall m\in[1\ldots M],$
\begin{equation}
    \left\langle\delta_{t_m}^+,g\ast\tilde\mu\right\rangle=\langle\delta_{t_m}^+,g\ast \mu\rangle,
\end{equation}
where $g=(\cdot)_+^0\e^{\alpha\cdot}$ is the Green's function of $(\Dd-\alpha\I).$ A calculation similar to that of Proposition \ref{prop:weakrep} shows that 
\begin{equation}
    \langle\delta_{t_m}^+,g\ast \mu\rangle=\int_{[K^-,t_m]}\e^{\alpha(t_m-x)}\mathrm{d}\mu(x),
\end{equation}
and that 
\begin{align}
\langle\delta_{t_m}^+,g\ast \tilde\mu\rangle=&\mu(\{t_1\})\int_{[K^-,t_m]}\e^{\alpha(t_m-x)}\,\mathrm{d}\delta_{t_1}+\sum_{m'=2}^{M-1}c_{m'}\int_{[K^-,t_{m'}]}\e^{\alpha(t_m-x)}\,\mathrm{d}\delta_{t_{m'}}\nonumber\\
=&\mu(\{t_1\})\int_{[K^-,t_m]}\e^{\alpha(t_m-x)}\,\mathrm{d}\delta_{t_1}+\sum_{m'=2}^{m}c_{m'}\int_{[K^-,t_m]}\e^{\alpha(t_m-x)}\,\mathrm{d}\delta_{t_{m'}}\nonumber\\
=&\mu(\{t_1\})\e^{\alpha(t_m-t_1)}+\sum_{m'=2}^{m}c_{m'}\e^{\alpha(t_m-t_{m'})}\nonumber\\
=&\mu(\{t_1\})\e^{\alpha(t_m-t_1)}+\sum_{m'=2}^{m}\e^{\alpha(t_m-t_{m'})}\int_{]t_{m'-1},t_{m'}]}\e^{\alpha(t_{m'}-x)}\,\mathrm{d}\mu(x)
\nonumber\\
=&\mu(\{t_1\})\e^{\alpha(t_m-t_1)}+\sum_{m'=2}^{m}\int_{]t_{m'-1},t_{m'}]}\e^{\alpha(t_{m}-x)}\,\mathrm{d}\mu(x)\nonumber\\
=&\int_{[t_1,t_m]}\e^{\alpha(t_{m}-x)}\,\mathrm{d}\mu(x).
§\end{align}
Consequently, it follows from \eqref{eq:4.2.105} and \eqref{eq:4.2.107} that $\mathcal{J}_{\omega}$ can only minimized if $\mathrm{supp}(\mu)\subset\{t_m\}_{m=1}^M$. In addition 
\begin{equation}
    \forall n\in[1,\ldots,N-1],\quad\langle(\Dd-\alpha\I)^{N-1,\star}\{\bm{\delta}_{\bb{t}}^+\}, p_n\rangle=0,\quad\text{and}\quad\norm{\mathrm{proj}_{\mathcal{N}_{\Ls}}\{p_n\}}_{\bb{p}}>0.
\end{equation}
Therefore,
\begin{equation}
    \mathcal{V}_{\omega}(\K)=\underset{f\in\Xi}{\mathrm{argmin}}\,\mathcal{J}_{\omega}(f),
\end{equation}
where 
\begin{equation}
    \Xi=\bigg\{ap_N+\sum_{m=1}^Ma_mg_{\Ls}(\cdot-t_m),\quad a\in\R,(a_m)_{m=1}^M\in\R^M\bigg\}
\end{equation}
is a vector space of dimension $(M+1)$. Consequently, $\mathcal{V}_{\omega}(\K)$ is nonempty. Next, observe that
\begin{equation}
   \langle(\Dd-\alpha\I)^{N-1,\star}\{\bm{\delta}_{\bb{t}}^+\}, p_N\rangle =\langle(\Dd-\alpha\I)^{N-1,\star}\{\bm{\delta}_{\bb{t}}^+\}, g_{\Ls}(\cdot-t_1)\rangle.
\end{equation}
Therefore, if $\lambda_1<\lambda_2$, then 
\begin{equation}
    \mathcal{V}_{\omega}(\K)=\underset{f\in\mathcal{X}}{\mathrm{argmin}}\,\mathcal{J}_{\omega}(f),
\end{equation}
where 
\begin{equation}
    \mathcal{X}=\bigg\{\sum_{m=1}^Ma_mg_{\Ls}(\cdot-t_m),\quad(a_m)_{m=1}^M\in\R^{M}\bigg\}
\end{equation}
is a vector space of dimension $M$. Since the functionals
\begin{equation}
    \Big(\langle(\Dd-\alpha\I)^{N-1,\star}\{\delta_{t_m}^+\}, p_N\rangle\Big)_{m=1}^M
\end{equation}
are linearly independant, the solution must be unique. The proof for the cases where $\lambda_1\geq \lambda_2$ is similar and omitted.
\end{proof}


\begin{Theorem}
\label{th:weakRT2}
Assume that Assumptions 1 to 3 hold and choose  $\epsilon$ small enough so that 
\begin{equation}
    t_{m-1}<t_m-\epsilon.
\end{equation} Let $\K_\epsilon^c:=\K\setminus\K_\epsilon$ and $\K_\epsilon$ be such that  
\begin{equation}
    \K_\epsilon:=\bigcup_{m=2}^{M}[t_{m}-\epsilon,t_m]\cup\{t_1\}
\end{equation}
If $\alpha<0$ and $\omega=0$, then the set $\mathcal{V}_{\omega}(\K_\epsilon)$ is nonempty and is the $\text{weak}^{\star}$-closed convex hull of its extreme points, which are of the form 
\begin{equation}
    c\frac{(\cdot-t_1)^{N-1}\e^{\alpha(\cdot-t_1)}}{(N-1)!}+\sum_{k=1}^{K}c_k\frac{(\cdot-x_k)^{N-1}_+\e^{\alpha(\cdot-x_k)}}{(N-1)!},\quad (\norm{c}_0+K)\leq M,\quad x_k\in\K_{\epsilon}.
\end{equation}
In addition, the following holds
\begin{equation}
    \lim_{\epsilon\to0}\mathcal{J}^{\star}_{\omega}(\K_{\epsilon})=\mathcal{J}^{\star}_{\omega}(\K).
\end{equation}
Finally, if $\mathcal{V}_\omega(\K)\neq\emptyset$, then there exists a unique solution 
\begin{equation}
f^{\star}(\cdot)=a(\cdot-t_1)^{N-1}\e^{\alpha(\cdot-t_1)}.
\end{equation}
\end{Theorem}

\begin{proof}[\textbf{Proof of Theorem \ref{th:weakRT2}}]
\hfill\\
\textbf{Step 1.} Let the sequence $(h_{\ell})_{\ell=1}^{\infty}$, with $h_{\ell}=p_{\ell}+g_{\Ls}\ast \mu_{\ell}\in\M_{\Ls}(\K)$, be such that 
\begin{equation}    \lim_{\ell\to\infty}\,\mathcal{J}_\omega(h_{\ell})=\mathcal{J}^{\star}_\omega(\K).
\end{equation}
Let $A_{\epsilon}=\bigcup_{m=2}^M[t_m-\epsilon,t_m]\cup\{t_1\}$ and define 
\begin{equation}
    f_{\ell}=p_{\ell}+g_{\Ls}\ast\tilde \mu_{\ell},\quad\text{with}\quad \tilde \mu_{\ell}=\mu_{\ell}\mathbbm{1}_{A_{\epsilon}}+\sum_{m=2}^{M}c_{\ell,m}\delta_{t_m-\epsilon}
\end{equation}
\begin{equation}
    c_m=\int_{]t_{m-1},t_{m}-\epsilon[}\e^{\alpha(t_m-x)}\,\mathrm{d}\mu(x).
\end{equation}
An argumentation similar to that of the proof of Theorem \ref{th:weakRT} shows that 
\begin{itemize}
    \item [1.] the following inequality holds $\norm{\Ls\{f_{\ell}\}}_{\M}\leq\norm{\Ls\{h_{\ell}\}}_{\M}$;
    \item [2.] the following inequality holds $\norm{\mathrm{proj}_{\mathcal{N}_{\Ls}}\{f_{\ell}\}}_{\bb{p}}\leq\norm{\mathrm{proj}_{\mathcal{N}_{\Ls}}\{h_{\ell}\}}_{\bb{p}}$;
    \item [3.] the following equality holds 
\begin{equation}
    \langle(\Dd-\alpha\I)^{N-1,\star}\{\bm{\delta}_{\bb{t}}^+\}, f_{\ell}\rangle=\langle(\Dd-\alpha\I)^{N-1,\star}\{\bm{\delta}_{\bb{t}}^+\},g_{\ell}\rangle.
\end{equation}
\end{itemize}
\end{proof}
